Impact of Noisy Supervision in Foundation Model Learning

Foundation models are usually pre-trained on large-scale datasets and then adapted to downstream tasks through tuning. However, the large-scale pre-training datasets, often inaccessible or too expensive to handle, can contain label noise that may adversely affect the generalization of the model and pose unexpected risks. This paper stands out as the first work to comprehensively understand and analyze the nature of noise in pre-training datasets and then effectively mitigate its impacts on downstream tasks. Specifically, through extensive experiments of fully-supervised and image-text contrastive pre-training on synthetic noisy ImageNet-1K, YFCC15M, and CC12M datasets, we demonstrate that, while slight noise in pre-training can benefit in-domain (ID) performance, where the training and testing data share a similar distribution, it always deteriorates out-of-domain (OOD) performance, where training and testing distributions are significantly different. These observations are agnostic to scales of pre-training datasets, pre-training noise types, model architectures, pre-training objectives, downstream tuning methods, and downstream applications. We empirically ascertain that the reason behind this is that the pre-training noise shapes the feature space differently. We then propose a tuning method (NMTune) to affine the feature space to mitigate the malignant effect of noise and improve generalization, which is applicable in both parameter-efficient and black-box tuning manners. We additionally conduct extensive experiments on popular vision and language models, including APIs, which are supervised and self-supervised pre-trained on realistic noisy data for evaluation. Our analysis and results demonstrate the importance of this novel and fundamental research direction, which we term as Noisy Model Learning.

==> tables/tb-ablation-mlp.tex <==
\begin{table}[h]
\centering
\caption{Ablation study of MLP architecture on ID tasks.}
\label{tab:ablation-mlp}
\resizebox{0.9 \linewidth}{!}{%
\begin{tabular}{@{}cc|c|c|c@{}}
\toprule
\multirow{2}{*}{MLP Layers} & \multirow{2}{*}{Activation} & \multirow{2}{*}{Noise (\%)} & IN-1K FS & YFCC15M CLIP \\
                   &                       &    & ID Accuracy & ID Accuracy \\ \midrule
\multirow{3}{*}{2} & \multirow{3}{*}{ReLU} & 0  &   75.06          &     67.34        \\
                   &                       & 5  &   74.87          &      67.44       \\
                   &                       & 10 &   74.27          &     66.95        \\ \midrule
\multirow{3}{*}{2} & \multirow{3}{*}{None} & 0  &   73.83          &      65.62       \\
                   &                       & 5  &   74.17         &        66.14     \\
                   &                       & 10 &   73.39          &       65.51      \\ \midrule
\multirow{3}{*}{3} & \multirow{3}{*}{ReLU} & 0  &    75.16         &     67.56        \\
                   &                       & 5  &     74.99        &     67.49        \\
                   &                       & 10 &     74.48        &     67.13        \\ \midrule
\multirow{3}{*}{4} & \multirow{3}{*}{ReLU} & 0  &     75.13        &     67.51        \\
                   &                       & 5  &     74.92        &      67.48       \\
                   &                       & 10 &     74.14  &            67.02 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/tb-ablation-weights.tex <==
\begin{table}[h]
\centering
\caption{Ablation study of loss weights on ID tasks. 
% \wjd{The left part is ugly: can we use \checkmark instead? The column ``Models'' should be ``Noise (\%)''}
}
\label{tab:ablation-loss}
\resizebox{0.9 \linewidth}{!}{%
\begin{tabular}{@{}ccc|c|c|c@{}}

\toprule
\multirow{2}{*}{$\mathcal{L}_{\mathrm{MSE}}$}  & \multirow{2}{*}{$\mathcal{L}_{\mathrm{COV}}$}  & \multirow{2}{*}{$\mathcal{L}_{\mathrm{SVD}}$}  & \multirow{2}{*}{Noise (\%)} & \multicolumn{1}{c|}{IN-1K FS} & YFCC15M CLIP \\
                      &                       &                       &    & \multicolumn{1}{c|}{ID Accuracy} & ID Accuracy \\ \midrule
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & 0                       &  75.06                  &     67.34                \\
                      &                       &                       & 5  &    74.87      &      67.44         \\
                      &                       &                       & 10 &  74.27        &      66.95       \\ \midrule
\multirow{3}{*}{} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & 0  &         74.34                       &       66.59   \\
                      &                       &                       & 5  &          74.18                         &       66.54      \\
                      &                       &                       & 10 &            74.09                    &     66.17        \\ \midrule
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & \multirow{3}{*}{\checkmark} & 0  &        73.65                          &      65.41     \\
                      &                       &                       & 5  &         74.23                           &     66.02       \\
                      &                       &                       & 10 &        73.56                          &     65.39        \\ \midrule
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & 0  &      74.74                            &        67.03     \\
                      &                       &                       & 5  &        74.32                       & 66.83            \\
                      &                       &                       & 10 &        73.92                         
 &        66.70     \\ \midrule
\multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & \multirow{3}{*}{} & 0  &       74.16                             &       66.27      \\
                      &                       &                       & 5  &        74.24                           &       66.31      \\
                      &                       &                       & 10 &        73.17                           &        66.08     \\ \midrule

\multirow{3}{*}{} & \multirow{3}{*}{\checkmark} & \multirow{3}{*}{} & 0  &       74.41                           &     66.51        \\
                      &                       &                       & 5  &        74.20                          &        66.47     \\
                      &                       &                       & 10 &           73.98                       &        66.12     \\ \midrule
\multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{\checkmark} & 0  &           72.21                       &      65.08       \\
                      &                       &                       & 5  &              73.49                    &     65.24        \\
                      &                       &                       & 10 &           72.87                       &       64.76      \\ \hline
\multirow{3}{*}{} & \multirow{3}{*}{} & \multirow{3}{*}{} & 0  &       73.96                           &       66.11      \\
                      &                       &                       & 5  &          73.97                        &     66.19        \\
                      &                       &                       & 10 &       73.13                           &     65.93        \\                       
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/tb-avg.tex <==
\begin{table}[t!]
    \begin{minipage}{.48\textwidth}
      \centering
        \caption{Results on popular vision models that are pre-trained on noisy datasets. We report the avarage accuracy on 14 in-domain (ID) and 4 out-of-domain (OOD) tasks. 
        % \wjd{Also: no std error?}
        }
        \label{tab:vision-res}
        \resizebox{\textwidth}{!}{
        % \begin{tabular}{l|l|l|cc|cc}
        \begin{tabular}{l|l|cc|cc}
        \toprule
        \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pre-trained \\ Model\end{tabular}}} &
          % \multicolumn{1}{c|}{\multirow{2}{*}{Model}} &
          \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tuning \\ Method\end{tabular}}} &
          \multicolumn{2}{c|}{In-Domain} &
          \multicolumn{2}{c}{Out-of-Domain} \\ \cline{3-6} 
        \multicolumn{1}{c|}{} &
          % \multicolumn{1}{c|}{} &
          \multicolumn{1}{c|}{} &
          Acc. &
          F1 &
          Acc. &
          F1 \\ \midrule
        \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}JFT300M\\ Semi-Supervised \\ EfficientNet-B3 \end{tabular}} &
          % \multirow{3}{*}{EfficientNet-B3} &
          LP &
          76.72 &
          0.3815 &
          44.13 &
          0.3594 \\
         &
           % &
          MLP &
          76.87 &
          0.3833 &
          45.95 &
          0.3624 \\
         &
           % &
          Ours &
          \textbf{77.63} &
          \textbf{0.3874} &
           \textbf{46.84} &
           \textbf{0.3654} \\ \midrule
        \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ImageNet-21K\\ Fully Supervised \\ ResNetv2-152x2 \end{tabular}} &
          % \multirow{3}{*}{ResNetv2-152x2} &
          LP &
          77.51 &
          0.3718 &
          40.82 &
          0.3062 \\
         &
           % &
          MLP &
          77.58 &
          0.3726 &
          41.73 &
          0.3053 \\
         &
           % &
          Ours &
          \textbf{78.43} &
          \textbf{0.3862} &
          \textbf{42.42} &
          \textbf{0.3100} \\ \midrule
        \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ImageNet-21K\\ Fully Supervised \\ Swin-L \end{tabular}} &
          % \multirow{3}{*}{Swin-L} &
          LP &
          81.91 &
          0.4092 &
          50.88 &
          0.3838 \\
         &
           % &
          MLP &
          82.51 &
          0.4128 &
          51.21 &
          0.3811 \\
         &
           % &
          Ours &
          \textbf{84.16} &
          \textbf{0.4177} &
          \textbf{52.35} &
          \textbf{0.3901} \\ \midrule
        \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Laion-2B\\ CLIP \\ ConvNext-L \end{tabular}} &
         %  \multirow{3}{*}{ConvNext-L} &
          LP &
          88.86 &
          0.4432 &
          66.86 &
          0.4253 \\
         &
          %  &
          MLP &
          88.53 &
          0.4417 &
          68.43 &
          0.4304 \\
         &
          % &
          Ours &
          \textbf{89.48} &
          \textbf{0.4457} &
          \textbf{70.30} &
           \textbf{0.4367} \\ \midrule
        \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Laion-2B\\ CLIP \\ ViT-L \end{tabular}} &
          % \multirow{3}{*}{ViT-L} &
          LP &
          86.85 &
          0.4328 &
          66.89 &
          0.4208 \\
         &
          % &
          MLP &
          87.23 &
          0.4375 &
          69.50 &
          0.4221 \\
         &
          % &
          Ours &
          \textbf{88.57} &
          \textbf{0.4414} &
          \textbf{70.47} &
          \textbf{0.4246} \\ 
        \bottomrule
        \end{tabular}%
        }%
    \end{minipage}%
    \hfill
    \begin{minipage}{.49\textwidth}
      \centering
        \caption{Evaluation of our method on language models in practice that are pre-trained on noisy datasets. We use GLUE for in-domain (ID) tasks and GLUE-X for out-of-domain (OOD) tasks.}
        \label{tab:nlp-results}
        \resizebox{0.85 \textwidth}{!}{%
        \begin{tabular}{@{}l|l|cc@{}}
        \toprule
        \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Pre-trained\\ Model\end{tabular}}} &
          \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Tuning\\ Method\end{tabular}}} &
          \multirow{2}{*}{In-Domain} &
          \multirow{2}{*}{Out-of-Domain} \\
        \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{} &  &  \\ \midrule
           % &                     & & \\
        \multirow{3}{*}{BERT-L}    & LP                    & 69.44 & 50.65 \\
                                   & MLP                   & 69.78 & 50.62 \\
                                   & Ours                  & \textbf{70.26} & \textbf{51.63} \\ \midrule
        \multirow{3}{*}{RoBERTa-L} & LP                    &  69.75 & 44.55 \\
                                   & MLP                   &  70.27 & 45.22 \\
                                   & Ours                  &  \textbf{70.97} &  \textbf{47.01} \\ \midrule
        \multirow{3}{*}{GPT-2}     & LP                    &  58.67 & 36.68 \\
                                   & MLP                   &  58.44 & 37.24 \\
                                   & Ours                  &  \textbf{59.34} &  \textbf{39.07} \\  \midrule
        \multirow{3}{*}{text-ada-002}     & LP               & 56.96 & 44.06 \\
                                   & MLP                   & 63.89 & 51.30  \\
                                   & Ours                  & \textbf{65.99} &  \textbf{53.48} \\ 
        \bottomrule
        \end{tabular}%
        }
    \end{minipage} 
\end{table}


==> tables/tb-cv-id.tex <==
\begin{table}[h]
\centering
\caption{Evaluation of our method on vision models in practice that are pre-trained on noisy datasets. We compare different methods on 14 vision datasets for in-domain (ID) evaluation}
\label{tab:res-cv-id}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|l|cccccccccccccc|c@{}}
\toprule
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Pre-trained \\ Model\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Tuning\\ Method\end{tabular}} &
  CIFAR10 &
  CIFAR100 &
  Flowers102 &
  Food101 &
  OxfordIIITPet &
  StanfordCars &
  FGVCAircraft &
  DTD &
  SVHN &
  Caltech101 &
  EuroSAT &
  PCAM &
  RESISC45 &
  RenderedSST2 &
  Avg \\  \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}JFT-300M \\ Semi-Supervised\\ EfficientNet-B3\end{tabular}} &
  LP &
  94.68$\pm$0.12 &
  79.00$\pm$0.23 &
  91.43$\pm$0.09 &
  79.71$\pm$1.02 &
  94.92$\pm$0.11 &
  59.36$\pm$0.98 &
  43.82$\pm$1.34 &
  73.60$\pm$0.20 &
  63.77$\pm$0.99 &
  \textbf{90.65$\pm$0.32} &
  95.88$\pm$0.01 &
  63.77$\pm$1.44 &
  89.62$\pm$0.87 &
  \textbf{53.93$\pm$0.23} &
  76.72 \\
 &
  MLP &
  95.87$\pm$0.08 &
  79.51$\pm$0.14 &
  87.78$\pm$0.53 &
  82.26$\pm$0.54 &
  94.96$\pm$0.11 &
  57.70$\pm$0.74 &
  41.46$\pm$2.42 &
  72.55$\pm$0.21 &
  \textbf{67.19$\pm$1.28} &
  87.52$\pm$0.58 &
  97.10$\pm$0.02 &
  \textbf{67.19$\pm$0.98} &
  92.25$\pm$0.54 &
  52.85$\pm$0.18 &
  76.87 \\
 &
  Ours &
  \textbf{96.15$\pm$0.05} &
  \textbf{79.71$\pm$0.10} &
  \textbf{91.61$\pm$0.09} &
  \textbf{82.63$\pm$0.51} &
  \textbf{95.29$\pm$0.13} &
  \textbf{60.24$\pm$0.69} &
  \textbf{43.57$\pm$1.02} &
  \textbf{73.78$\pm$0.18} &
  67.05$\pm$0.54 &
  88.73$\pm$0.44 &
  \textbf{97.20$\pm$0.01} &
  67.05$\pm$0.91 &
  \textbf{92.60$\pm$0.40} &
  51.25$\pm$0.08 &
  \textbf{77.63} \\  \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ImageNet-21K\\ Fully Supervised\\ ResNetv2-152x2\end{tabular}} &
  LP &
  96.39$\pm$0.13 &
  85.21$\pm$0.17 &
  96.85$\pm$0.08 &
  85.99$\pm$0.47 &
  91.73$\pm$0.20 &
  55.96$\pm$1.23 &
  43.37$\pm$0.98 &
  73.51$\pm$0.55 &
  62.51$\pm$0.83 &
  \textbf{92.15$\pm$0.16} &
  97.15$\pm$0.13 &
  58.70$\pm$0.87 &
  92.20$\pm$0.43 &
  53.47$\pm$0.32 &
  77.51 \\
 &
  MLP &
  97.02$\pm$0.11 &
  85.47$\pm$0.19 &
  96.96$\pm$0.09 &
  \textbf{86.46$\pm$0.34} &
  92.39$\pm$0.23 &
  57.25$\pm$1.12 &
  41.10$\pm$1.45 &
  73.76$\pm$0.43 &
  64.61$\pm$0.56 &
  89.50$\pm$0.21 &
  97.59$\pm$0.11 &
  59.66$\pm$0.45 &
  93.33$\pm$0.27 &
  51.02$\pm$0.59 &
  77.58 \\
 &
  Ours &
  \textbf{97.12$\pm$0.11} &
  \textbf{85.68$\pm$0.16} &
  \textbf{96.98$\pm$0.08} &
  85.69$\pm$0.35 &
  \textbf{92.49$\pm$0.18} &
  \textbf{57.42$\pm$0.99} &
  \textbf{43.54$\pm$1.23} &
  \textbf{73.87$\pm$0.46} &
  \textbf{66.94$\pm$0.50} &
  92.01$\pm$0.12 &
  \textbf{97.67$\pm$0.09} &
  \textbf{61.12$\pm$0.41} &
  \textbf{93.97$\pm$0.35} &
  \textbf{53.53$\pm$0.71} &
  \textbf{78.43} \\  \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ImageNet-21K\\ Fully Supervised\\ Swin-L\end{tabular}} &
  LP &
  98.06$\pm$0.07 &
  88.51$\pm$0.12 &
  99.27$\pm$0.04 &
  89.68$\pm$0.63 &
  92.60$\pm$0.19 &
  65.43$\pm$0.34 &
  53.48$\pm$1.44 &
  77.45$\pm$0.39 &
  72.94$\pm$0.33 &
  \textbf{90.91$\pm$0.09} &
  97.00$\pm$0.50 &
  72.94$\pm$0.23 &
  93.84$\pm$0.21 &
  54.59$\pm$0.70 &
  81.91 \\
 &
  MLP &
  98.45$\pm$0.06 &
  89.72$\pm$0.09 &
  99.12$\pm$0.05 &
  91.20$\pm$0.30 &
  93.75$\pm$0.24 &
  68.15$\pm$1.22 &
  52.81$\pm$0.78 &
  77.63$\pm$0.42 &
  73.48$\pm$0.32 &
  89.26$\pm$0.22 &
  \textbf{98.07$\pm$0.10} &
  74.48$\pm$0.37 &
  95.04$\pm$0.23 &
  54.09$\pm$0.52 &
  82.52 \\
 &
  Ours &
  \textbf{98.60$\pm$0.06} &
  \textbf{90.14$\pm$0.11} &
  \textbf{99.53$\pm$0.03} &
  \textbf{91.40$\pm$0.33} &
  \textbf{94.22$\pm$0.22} &
  \textbf{75.60$\pm$2.12} &
  \textbf{55.95$\pm$0.91} &
  \textbf{79.97$\pm$0.20} &
  \textbf{76.61$\pm$0.12} &
  90.36$\pm$0.26 &
  98.06$\pm$0.11 &
  \textbf{76.61$\pm$0.41} &
  \textbf{95.34$\pm$0.23} &
  \textbf{55.92$\pm$0.48} &
  \textbf{84.17} \\  \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Laion-2B\\ CLIP\\ ConvNext-L\end{tabular}} &
  LP &
  98.15$\pm$0.08 &
  88.83$\pm$0.24 &
  \textbf{98.72$\pm$0.12} &
  91.68$\pm$0.28 &
  94.07$\pm$0.15 &
  94.68$\pm$0.33 &
  65.94$\pm$0.45 &
  \textbf{83.88$\pm$0.04} &
  82.41$\pm$0.21 &
  \textbf{96.37$\pm$0.03} &
  97.78$\pm$0.01 &
  82.41$\pm$0.21 &
  95.44$\pm$0.05 &
  73.70$\pm$0.10 &
  88.86 \\
 &
  MLP &
  98.64$\pm$0.05 &
  89.67$\pm$0.18 &
  96.35$\pm$0.47 &
  92.80$\pm$0.41 &
  93.55$\pm$0.13 &
  94.47$\pm$0.32 &
  67.06$\pm$0.75 &
  81.33$\pm$0.24 &
  82.08$\pm$0.45 &
  94.33$\pm$0.02 &
  98.22$\pm$0.03 &
  82.25$\pm$0.15 &
  96.51$\pm$0.14 &
  72.27$\pm$0.14 &
  88.54 \\
 &
  Ours &
  \textbf{98.73$\pm$0.06} &
  \textbf{90.39$\pm$0.14} &
  98.50$\pm$0.26 &
  \textbf{92.90$\pm$0.24} &
  \textbf{94.52$\pm$0.12} &
  \textbf{95.48$\pm$0.19} &
  \textbf{69.18$\pm$0.51} &
  83.23$\pm$0.19 &
  \textbf{82.83$\pm$0.17} &
  95.26$\pm$0.05 &
  \textbf{98.46$\pm$0.03} &
  \textbf{82.53$\pm$0.15} &
  \textbf{96.82$\pm$0.08} &
  \textbf{73.94$\pm$0.23} &
  \textbf{89.48} \\  \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Laion-2B\\ CLIP\\ ViT-L\end{tabular}} &
  LP &
  98.09$\pm$0.05 &
  88.43$\pm$0.25 &
  95.89$\pm$0.11 &
  91.67$\pm$0.50 &
  93.24$\pm$0.09 &
  93.04$\pm$0.34 &
  62.28$\pm$1.23 &
  81.70$\pm$0.23 &
  77.02$\pm$0.58 &
  93.44$\pm$0.09 &
  97.28$\pm$0.02 &
  77.02$\pm$1.25 &
  95.86$\pm$0.31 &
  71.00$\pm$0.50 &
  86.85 \\ 
 &
  MLP &
  97.52$\pm$0.14 &
  88.33$\pm$0.34 &
  95.54$\pm$0.40 &
  92.12$\pm$0.36 &
  93.41$\pm$0.09 &
  93.34$\pm$0.31 &
  63.11$\pm$0.84 &
  81.97$\pm$0.15 &
  77.81$\pm$0.64 &
  92.35$\pm$0.15 &
  97.38$\pm$0.01 &
  79.11$\pm$0.35 &
  96.54$\pm$0.05 &
  72.74$\pm$0.51 &
  87.23 \\
  & 
  Ours &
  \textbf{98.65$\pm$0.05} &
  \textbf{88.96$\pm$0.22} &
  \textbf{98.67$\pm$0.15} &
  \textbf{92.78$\pm$0.27} &
  \textbf{94.51$\pm$0.10} &
  \textbf{94.65$\pm$0.52} &
  \textbf{67.29$\pm$0.47} &
  \textbf{82.98$\pm$0.14} &
  \textbf{79.25$\pm$0.72} &
  \textbf{93.65$\pm$0.08} &
  \textbf{98.59$\pm$0.03} &
  \textbf{79.35$\pm$0.30} &
  \textbf{97.19$\pm$0.19} &
  \textbf{73.51$\pm$0.43} &
  \textbf{88.57} \\
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/tb-cv-ood.tex <==
\begin{table}[h]
\centering
\caption{Evaluation of our method on vision models in practice that are pre-trained on noisy datasets. We compare different methods on 4 DomainNet datasets for out-of-domain (OOD) evaluation. We perform training on either DomainNetSketch or DomainNetReal, and evaluate on DomainNetSketch, DomainNetReal, DomainNetPaining, DomainNetClipart without the training set. }
\label{tab:res-cv-ood}
\resizebox{0.5 \textwidth}{!}{%
\begin{tabular}{@{}l|l|ccc@{}}
\toprule
\multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Pre-trained \\ Model\end{tabular}} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Tuning\\ Method\end{tabular}} &
  DomainNet Sketch &
  DomainNet Real &
  Avg \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}JFT-300M \\ Semi-Supervised\\ EfficientNet-B3\end{tabular}} &
  LP &
  46.22$\pm$6.17 &
  42.03$\pm$7.07 &
  44.13 \\
 &
  MLP &
  48.29$\pm$5.78 &
  43.61$\pm$7.53 &
  45.95 \\
 &
  Ours &
  \textbf{48.84$\pm$5.63} &
  \textbf{44.83$\pm$7.45} &
  \textbf{46.84} \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ImageNet-21K\\ Fully Supervised\\ ResNetv2-152x2\end{tabular}} &
  LP &
  41.09$\pm$4.81 &
  40.55$\pm$7.89 &
  40.82 \\
 &
  MLP &
  41.98$\pm$5.08 &
  41.47$\pm$7.45 &
  41.73 \\
 &
  Ours &
  \textbf{42.68$\pm$4.85} &
  \textbf{42.15$\pm$7.23} &
  \textbf{42.42} \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}ImageNet-21K\\ Fully Supervised\\ Swin-L\end{tabular}} &
  LP &
  54.57$\pm$7.70 &
  47.19$\pm$7.45 &
  50.88 \\
 &
  MLP &
  53.81$\pm$6.01 &
  48.60$\pm$8.12 &
  51.21 \\
 &
  Ours &
  \textbf{55.68$\pm$5.48} &
  \textbf{49.01$\pm$6.15} &
  \textbf{52.35} \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Laion-2B\\ CLIP\\ ConvNext-L\end{tabular}} &
  LP &
  66.66$\pm$7.69 &
  67.05$\pm$4.58 &
  66.86 \\
 &
  MLP &
  66.78$\pm$7.00 &
  70.07$\pm$4.90 &
  68.43 \\
 &
  Ours &
  \textbf{69.74$\pm$6.82} &
  \textbf{70.85$\pm$4.77} &
  \textbf{70.30} \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Laion-2B\\ CLIP\\ ViT-L\end{tabular}} &
  LP &
  67.00$\pm$6.94 &
  66.77$\pm$4.74 &
  66.89 \\
 &
  MLP &
  68.99$\pm$6.59 &
  70.00$\pm$4.65 &
  69.50 \\
 &
  Ours &
  \textbf{70.48$\pm$6.91} &
  \textbf{70.45$\pm$4.98} &
  \textbf{70.47}
  \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/tb-id-dataset.tex <==
\begin{table}[t!]
\centering
\caption{Details of the 14 in-domain (ID) vision datasets used to evaluate ID transfer performance of vision models.}
\label{tab:append-exp-vision-id}
\resizebox{0.9\linewidth}{!}{%
\begin{tabular}{l|cccc}
\toprule
\multicolumn{1}{c|}{Dataset} &  Classes & Train Size & Test Size & Evaluation Metric \\ \hline
CIFAR-10 \cite{krizhevsky2009learning}                    &            10 & 50,000 & 10,000   & accuracy           \\ 
CIFAR-100  \cite{krizhevsky2009learning}                   &          100 & 50,000 & 10,000    & accuracy                     \\
Flowers102 \cite{nilsback2008automated}               &       102 & 2,040 & 6,149            & mean per class       \\ 
Food101 \cite{FeiFei2004LearningGV}                    &    101 & 75,750 & 25,250       & accuracy               \\ 
OxfordPet \cite{parkhi12a}                    &           37 & 3,680 & 3,669          & mean per class            \\
StanfordCars  \cite{jonathan2013cars}              &       196 & 8,144 & 8,041         & accuracy              \\ 
FGVCAircraft  \cite{maji2013finegrained}              &    102 & 6,667 & 3,333         & mean per class               \\ 
SVHN  \cite{2011svhn}              &           10 & 73,257 & 26,032   & accuracy     \\ 
DTD  \cite{cimpoi14describing}              &          47 & 1,880 & 1,880           & accuracy        \\ 
Caltech101  \cite{FeiFei2004LearningGV}              &     102 & 3,060 & 6,084       & mean per class               \\ 
EuroSAT  \cite{helber2019eurosat}              &     10 & 21,600 & 5,400       & accuracy            \\ 
PatchCamelyon  \cite{Veeling2018qh}              &      10 & 73,257 & 26,032     & accuracy     \\ 
RESISC45  \cite{Cheng2017resic}              &          45 & 25,200 & 6,300       & accuracy                \\ 
Rendered SST2  \cite{socher2013recursive}              &     2 & 6,920 & 1,821         & accuracy                 \\ 
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/tb-nlp-id.tex <==
% {\floatsetup[table]{capposition=top}
\begin{table}[t!]
\centering
\caption{Evaluation of our method on language models in practice that are pre-trained on noisy datasets. We compare different methods on GLUE dev set for in-domain (ID) evaluation.}
\label{tab:res-nlp-id}
\resizebox{0.9 \textwidth}{!}{%
\begin{tabular}{@{}l|l|ccccccccl@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Model}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{Tuning}} &
  CoLA &
  MNLI &
  MRPC &
  QNLI &
  QQP &
  RTE &
  SST2 &
  STS &
  \multicolumn{1}{c}{\multirow{2}{*}{Avg}} \\
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  MCC &
  Acc &
  Acc &
  Acc &
  Acc &
  Acc &
  Acc &
  PCC &
  \multicolumn{1}{c}{} \\ \midrule
\multirow{3}{*}{BERT-L} &
  LP &
  46.18 &
  62.75 &
  72.05 &
  74.10 &
  84.83 &
  50.90 &
  88.19 &
  76.55 &
  69.44 \\
 &
  MLP &
  \textbf{46.99} &
  63.97 &
  72.30 &
  73.80 &
  84.88 &
  51.62 &
  88.30 &
  76.36 &
  69.78 \\
 &
  Ours &
  46.12 &
  \textbf{64.37} &
  \textbf{73.04} &
  \textbf{74.25} &
  \textbf{85.11} &
  \textbf{52.54} &
  \textbf{88.84} &
  \textbf{76.64} &
  \textbf{70.26} \\ \midrule
\multirow{3}{*}{RoBERTa-L} &
  LP &
  41.09 &
  59.27 &
  76.47 &
  76.07 &
  83.19 &
  55.96 &
  90.02 &
  75.93 &
  69.76 \\
 &
  MLP &
  42.93 &
  60.38 &
  76.22 &
  76.11 &
  82.94 &
  57.40 &
  90.25 &
  75.92 &
  70.27 \\
 &
  Ours &
  \textbf{43.91} &
  \textbf{60.59} &
  \textbf{77.69} &
  \textbf{76.33} &
  \textbf{83.30} &
  \textbf{58.96} &
  \textbf{90.71} &
  \textbf{76.24} &
  \textbf{70.97} \\ \midrule
\multirow{3}{*}{GPT-2} &
  LP &
  4.86 &
  53.11 &
  72.55 &
  67.65 &
  78.82 &
  56.68 &
  84.75 &
  40.93 &
  57.42 \\
 &
  MLP &
  4.46 &
  53.38 &
  73.53 &
  67.17 &
  78.72 &
  56.68 &
  84.75 &
  40.93 &
  57.19 \\
 &
  Ours &
  \textbf{6.41} &
  \textbf{54.21} &
  \textbf{73.77} &
  \textbf{68.09} &
  \textbf{78.95} &
  \textbf{57.07} &
  \textbf{85.14} &
  \textbf{41.09} &
  \textbf{58.09} \\ 
\midrule
\multirow{3}{*}{text-ada-002} &
  LP &
  22.92 &
  69.85 &
  64.74 &
  62.14 &
  74.96 &
  51.98 &
  91.05 &
  18.04 &
  56.96 \\
 &
  MLP &
  33.90 &
  70.49 &
  66.42 &
  69.54 &
  84.28 &
  52.34 &
  91.85 &
  42.28 &
  63.89 \\
 &
  Ours &
  \textbf{36.96} &
  \textbf{72.05} &
  \textbf{70.34} &
  \textbf{70.25} &
  \textbf{85.54} &
  \textbf{54.51} &
  \textbf{92.89} &
  \textbf{45.39} &
  \textbf{65.99} \\ 

\bottomrule
\end{tabular}%
}
\end{table}

==> tables/tb-nlp-models.tex <==
\begin{table}[t]
\centering
\caption{Noisy language models details. \wjd{why no param size? what is ``and d English''?}}
\label{tab:nlp-model-details}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{@{}ccc@{}}
\toprule
Model & Pre-trained Data & Pre-trained Method \\ \midrule
BERT-L \cite{devlin2018bert}      &    BooksCorpus and d English Wikipedia            &      Masked Modeling \cite{devlin2018bert}                      \\
RoBERTa-L \cite{liu2019roberta}     &     BooksCorpus and d English Wikipedia        &               Masked Modeling  \cite{liu2019roberta}           \\ 
GPT-2  \cite{radford2019language} &       WebText        &      Autoregression        \\ 
text-ada-002     &          -  &            -         \\ 
\bottomrule
\end{tabular}%
}
\vspace{-0.1in}
\end{table}

==> tables/tb-nlp-ood.tex <==
% {\floatsetup[table]{capposition=top}
\begin{table}[t!]
\centering
\caption{Evaluation of our method on language models in practice that are pre-trained on noisy datasets. We compare different methods on GLUE-X for ouf-of-domain (OOD) evaluation.}
\label{tab:res-nlp-ood}
\resizebox{0.9 \textwidth}{!}{%
\begin{tabular}{@{}l|l|ccccccccl@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Model}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{Tuning}} &
  CoLA &
  MNLI &
  MRPC &
  QNLI &
  QQP &
  RTE &
  SST2 &
  STS &
  \multicolumn{1}{c}{\multirow{2}{*}{Avg}} \\
\multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{} &
  MCC &
  Acc &
  Acc &
  Acc &
  Acc &
  Acc &
  Acc &
  PCC &
  \multicolumn{1}{c}{} \\ \midrule
\multirow{3}{*}{BERT-L} &
  LP &
  13.71 &
  36.82 &
  55.85 &
  63.60 &
  53.14 &
  50.67 &
  73.66 &
  57.81 &
  50.65 \\
 &
  MLP &
  14.11 &
  36.49 &
  56.15 &
  63.61 &
  52.34 &
  50.02 &
  73.32 &
  58.91 &
  50.62 \\
 &
  Ours &
  \textbf{14.57} &
  \textbf{37.62} &
  \textbf{56.68} &
  \textbf{63.88} &
  \textbf{55.17} &
  \textbf{50.98} &
  \textbf{74.52} &
  \textbf{59.61} &
  \textbf{51.63} \\ \midrule
\multirow{3}{*}{RoBERTa-L} &
  LP &
   24.07  &
   37.05 &
   48.51 &
   57.83 &
   24.93 &
   51.02 &
   71.24 &
   41.74 &
   44.55 \\
 &
  MLP &
  24.50 &
  37.32 &
  48.96 &
  58.56 &
  24.12 &
  52.51 &
  73.86 &
  41.95 &
  45.22 \\
  &
  Ours &
  \textbf{25.29} &
  \textbf{37.84} &
  \textbf{49.52} &
  \textbf{59.72} &
  \textbf{26.78} &
  \textbf{53.19} &
  \textbf{81.42} &
  \textbf{42.29} &
  \textbf{47.01} \\ \midrule
\multirow{3}{*}{GPT-2} &
  LP &
  4.12 &
  24.93 &
  45.24 &
  54.00 &
  16.22 &
  49.50 &
  53.75 &
  45.68 &
  36.68 \\
 &
  MLP &
  4.89 &
  25.20 &
  47.99 &
  54.11 &
  17.21 &
  49.71 &
  53.60 &
  45.21 &
  37.24 \\
 &
  Ours &
  \textbf{5.31} &
  \textbf{32.56} &
  \textbf{49.78} &
  \textbf{55.97} &
  \textbf{17.34} &
  \textbf{49.96} &
  \textbf{54.28} &
  \textbf{47.39} &
  \textbf{39.07} \\ 
\midrule
\multirow{3}{*}{text-ada-002} &
  LP &
   8.06 &
   65.14&
   38.66 &
   58.12 &
   32.60 &
   51.53 &
   84.07 &
   14.30 &
   44.06 \\
 &
  MLP &
   15.47 &
   67.23 &
   44.91 &
   63.59 &
   50.24 &
   51.44 &
   83.11 &
   34.46 &
   51.31 \\
 &
  Ours &
  \textbf{17.50} &
  \textbf{68.97} &
  \textbf{46.41} &
  \textbf{63.81} &
  \textbf{55.34} &
  \textbf{52.81} &
  \textbf{85.16} &
  \textbf{37.80} &
  \textbf{53.48} \\ 

\bottomrule
\end{tabular}%
}
\end{table}

==> tables/tb-ood-dataset.tex <==
\begin{table}[t!]
\centering
\caption{Details of the 4 out-of-domain (OOD) DomainNet and 6 ImageNet variants datasets used to evaluate OOD transfer performance of vision models.}
\label{tab:append-exp-vision-odd}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{l|cccc}
\toprule
\multicolumn{1}{c|}{Dataset} & Classes & Train Size & Test Size & Evaluation Metric \\ \hline
DomainNet Sketch \cite{peng2019moment}                            &          345 & 48,212 & 20,916                   & accuracy              \\ 
DomainNet Real \cite{peng2019moment}                              &      345 & 120,906 & 52,041                   &       accuracy          \\
DomainNet Painting \cite{peng2019moment}                         &           345 & - & 21,850                 &        accuracy        \\ 
DomainNet Clipart \cite{peng2019moment}                         &         345 & - & 14,604                  &            accuracy     \\ \hline
ImageNet-V2 \cite{recht2019imagenet}                         &        1,000             &     -     &     10,000                &        accuracy          \\ 
ImageNet-R \cite{dan2021ood}                  &              200       &               -  &            30,000        &           accuracy \\ 
ImageNet-Sketch \cite{wang2019learning}                         &   1,000                  &      -   &      50,889               &             accuracy      \\ 
ImageNet-A \cite{dan2021ood}                           &     200                &           -   &       7,500              &          accuracy    \\ 
ImageNet-ViD \cite{vaishaal2021time}                           &    1,000                 &     -    &  \ch{fill this}                   &            accuracy       \\ 
ObjectNet \cite{objectnet2019}                               &      112               &        -    &       18,574              &         accuracy       \\ 
\bottomrule
\end{tabular}%
}
\end{table}

==> tables/tb-seg.tex <==
\begin{table}[t!]
\centering
\caption{Instance segmentation results on COCO 2017 of IN-1K ResNet-50 noisy FS pre-trained models.}
\label{tab:r50_seg}
\resizebox{0.75 \columnwidth}{!}{%
\begin{tabular}{@{}c|c|ccc@{}}
\toprule
Segmentation & Noise (\%) & \multicolumn{1}{c}{$\textrm{AP}^{\textrm{mask}}$} & \multicolumn{1}{c}{$\textrm{AP}^{\textrm{mask}}_{50}$} & \multicolumn{1}{c}{$\textrm{AP}^{\textrm{mask}}_{75}$} \\ \midrule
\multirow{5}{*}{Mask R-CNN \cite{he2017mask}} & 0  & 31.3 & \textbf{51.3} & 33.0 \\
                              & 5  & \textbf{31.4} & \textbf{51.3} & \textbf{33.2} \\
                              & 10 & \textbf{31.3} & \textbf{51.3}   & 32.9 \\
                              & 20 & 31.2 & 51.1 & 32.8 \\
                              & 30 & 30.30 & 49.9 & 32.1 \\ \midrule
\multirow{5}{*}{SOLOv2 \cite{wang2020solov2}}     & 0  & 32.2 & 52.7 & 33.6 \\
                              & 5  & \textbf{32.7} & \textbf{53.2} & \textbf{34.2} \\
                              & 10 & 32.4 & 52.8 & 33.9 \\
                              & 20 & 32.0 & 52.2 & 33.6 \\
                              & 30 & 31.4   & 51.3 & 32.5 \\ \bottomrule
\end{tabular}%
}
\end{table}
